Quantum Link Homology via Trace Functor I

Motivated by topology, we develop a general theory of traces and shadows for an endobicategory, which is a~pair: bicategory $\mathbf{C}$ and endobifunctor $\Sigma\colon \mathbf C \to\mathbf C$. For a graded linear bicategory and a fixed invertible parameter $q$, we quantize this theory by using the endofunctor $\Sigma_q$ such that $\Sigma_q \alpha:=q^{-\deg \alpha}\Sigma\alpha$ for any 2-morphism $\alpha$ and coincides with $\Sigma$ otherwise. Applying the quantized trace to the~bicategory of Chen-Khovanov bimodules we get a new triply graded link homology theory called quantum annular link homology. If $q=1$ we reproduce Asaeda-Przytycki-Sikora (APS) homology for links in a thickened annulus. We prove that our homology carries an action of $\mathcal U_q(\mathfrak{sl}_2)$, which intertwines the action of cobordisms. In particular, the~quantum annular homology of an $n$-cable admits an action of the braid group, which commutes with the quantum group action and factors through the Jones skein relation. This produces a nontrivial invariant for surfaces knotted in four dimensions. Moreover, a direct computation for torus links shows that the rank of quantum annular homology groups does depend on the quantum parameter $q$.

==> macros.tex <==
\def\Span{\mathrm{span}}
\def\grep{\mathrm{gRep}(\LieSL_2)}
\def\qrep{\mathrm{gRep}_q(\LieSL_2)}

\makeatletter

% =======================================================================================
%  Creating repeated theorems
%
%  Example: to put a formulation of Theorem 7.4, which is the main result, in the
%           introduction of the paper.
%
%  \begin{repeattheorem}{Theorem}{thm:main-result}
%     (here goes the formulation of the theorem)
%  \end{repeattheorem}
%
%  (somewhere in section 7)
%
%  \begin{theorem}\label{thm:main-result}
%     (here goes the formulation of the theorem)
%  \end{theorem}
%
% =======================================================================================

\newcount\repeatedID
\repeatedID=0
\def\repeattheorem#1#2{%
	\theoremstyle{plain}
	\newtheorem*{RepeatedTheorem\the\repeatedID}{#1~\ref{#2}}%
	\begin{RepeatedTheorem\the\repeatedID}%
}
\def\endrepeattheorem{%
	\end{RepeatedTheorem\the\repeatedID}%
	\global\advance\repeatedID 1\relax
}
 
% =======================================================================================
%  Drawing commands
% =======================================================================================

\definecolor{annulus}{rgb}{0.97,0.97,0.97}

\def\drawinannulus{\@ifnextchar({\drawinannulus@at}{\drawinannulus@at(0,0)}}
\def\drawinannulus@at(#1){\@ifnextchar[{\drawinannulus@(#1)}{\drawinannulus@(#1)[3,1]}}
\def\drawinannulus@(#1)[#2,#3]#4{\begingroup
	\psset{linewidth=0.5pt,dimen=inner,fillstyle=solid}%
	\psclip{\pscircle[fillcolor=annulus](#1){#2}}\psset{linewidth=1pt}\SpecialCoor#4\endpsclip
	\pscircle[fillcolor=white](#1){#3}%
\endgroup}

\def\coupon(#1)#2{%
	\rput(#1){\psframebox*[framesep=2pt]{\phantom{$\scriptstyle#2$}}}%
	\rput(#1){\psframebox[framearc=0.5,framesep=2pt]{%
		\vphantom{$\scriptstyle#2$}\smash{\raisebox{-0.5pt}{$\scriptstyle#2$}}}}%
}%


% =======================================================================================
%  Generating links for arXiv references
% =======================================================================================

\def\arXiv#1{\arXiv@#1.}
\def\arXiv@#1.#2#3#4#5.{%
	\ifx\relax#5\relax
		\href{http://front.math.ucdavis.edu/#1.5#2#3#4}{arXiv:math/#1#2#3#4}%
	\else
		\href{http://front.math.ucdavis.edu/#1.#2#3#4#5}{arXiv:#1.#2#3#4#5}%
	\fi
}

% =======================================================================================
%  Lowering accents over symbols
% =======================================================================================

\def\lowtilde{\@ifnextchar[{\lowtilde@}{\lowtilde@[1.2]}}%
\def\lowtilde@[#1]#2{%
	\mathchoice
		{\lthelper\textfont\displaystyle{#1}{#2}}%
		{\lthelper\textfont\textstyle{#1}{#2}}%
		{\lthelper\scriptfont\scriptstyle{#1}{#2}}%
		{\lthelper\scriptscriptfont\scriptscriptstyle{#1}{#2}}%
}
\def\lthelper#1#2#3#4{%
	\hbox{%
		\dimen@\accentfontxheight#1%
		\accentfontxheight#1#3\dimen@
		$\m@th#2\widetilde{#4}$%
		\accentfontxheight#1\dimen@
	}%
}

\def\accentfontxheight#1{%
	\fontdimen5#13
}
\makeatother


% =======================================================================================
%  Visualization of Hochschild chains
% =======================================================================================

\def\HCsegments#1,{%
	\ifx\relax#1\relax\else
		\psline(1.4em;#1)(2.1em;#1)%
		\expandafter\HCsegments
	\fi}%
\def\HClabels#1@#2,{%
	\ifx\relax#2\relax\else
		\rput*(1.75em;#2){$#1$}%
		\expandafter\HClabels
	\fi}%

\makeatletter
\def\HochschildChain{%
	\@ifnextchar(\HochschildChainMembrane
		{\HochschildChainMembrane(-3.5em,-1.75em)(3.5em,1.75em)}}%
\def\HochschildChainMembrane(#1)(#2){%
	\@ifnextchar[{\HochschildChainDraw(#1)(#2)}%
	             {\HochschildChainDraw(#1)(#2)[]}}%
\makeatother

\def\HochschildChainDraw(#1)(#2)[#3]#4#5{%
	\begin{centerpict}(#1)(#2)
		\SpecialCoor
		\pscircle(0,0){1.75em}
		\HCsegments#4,\relax,%
		\ifx\relax#3\relax\else
			\psline[linecolor=blue,linewidth=4pt](1.3em;#3)(2.2em;#3)%
		\fi
		\HClabels#5,@\relax,%
	\end{centerpict}}

% =======================================================================================
%  Miscallenous
% =======================================================================================

\def\genericmatrix#1#2(#3,#4){\begin{#1}
	#2_{11} & \cdots & #2_{1#3} \\
	\vdots  & \ddots & \vdots   \\
	#2_{#41}& \cdots & #2_{#4#3}\\
\end{#1}}
\def\gmatrix{\genericmatrix{pmatrix}}
\def\gsmallmatrix{\genericmatrix{psmallmatrix}}

